Beam Aware Stochastic Multihop Routing for Flying Ad-hoc Networks

Routing is a crucial component in the design of Flying Ad-Hoc Networks (FANETs). State of the art routing solutions exploit the position of Unmanned Aerial Vehicles (UAVs) and their mobility information to determine the existence of links between them, but this information is often unreliable, as the topology of FANETs can change quickly and unpredictably. In order to improve the tracking performance, the uncertainty introduced by imperfect measurements and tracking algorithms needs to be accounted for in the routing. Another important element to consider is beamforming, which can reduce interference, but requires accurate channel and position information to work. In this work, we present the Beam Aware Stochastic Multihop Routing for FANETs (BA-SMURF), a Software-Defined Networking (SDN) routing scheme that takes into account the positioning uncertainty and beamforming design to find the most reliable routes in a FANET. Our simulation results show that joint consideration of the beamforming and routing can provide a 5% throughput improvement with respect to the state of the art.

==> Images/results/boxplots/boxplot_density10.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.8\linewidth,
height=1.0in,
at={(0.5in,1.5in)},
scale only axis,
xmin=0.5,
xmax=6.5,
xtick={1,2,3,4,5,6},
xticklabels={{SMURF-T}, {DBR-T}, {BASMURF-T},{SMURF},{DBR},{BASMURF}},
xticklabel style={rotate=45},
ymin=740727934.615314,
ymax=938075750.865038,
ylabel style={font=\color{white!15!black}},
ylabel={average throughput},
xlabel={(a) $Density=25000~UAVs/km^3$},
axis background/.style={fill=white},
title style={font=\bfseries},
title={}
]
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	792198135.497689\\
1	820192059.578569\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	790444965.139975\\
2	811485121.51285\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	797440093.455926\\
3	824610155.741313\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	874920787.999411\\
4	897436595.580075\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	873518182.255416\\
5	895132688.343446\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	880909562.089288\\
6	908068570.845574\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	749698289.899392\\
1	771319845.175757\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	767572741.830301\\
2	775610905.379772\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	751077624.986745\\
3	778811518.589989\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	834298735.531422\\
4	855321034.77516\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	852521520.47077\\
5	857650560.681162\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	836438997.950208\\
6	861788099.394419\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	820192059.578569\\
1.125	820192059.578569\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	811485121.51285\\
2.125	811485121.51285\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	824610155.741313\\
3.125	824610155.741313\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	897436595.580075\\
4.125	897436595.580075\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	895132688.343446\\
5.125	895132688.343446\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	908068570.845574\\
6.125	908068570.845574\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	749698289.899392\\
1.125	749698289.899392\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	767572741.830301\\
2.125	767572741.830301\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	751077624.986745\\
3.125	751077624.986745\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	834298735.531422\\
4.125	834298735.531422\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	852521520.47077\\
5.125	852521520.47077\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	836438997.950208\\
6.125	836438997.950208\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
0.75	771319845.175757\\
0.75	792198135.497689\\
1.25	792198135.497689\\
1.25	771319845.175757\\
0.75	771319845.175757\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
1.75	775610905.379772\\
1.75	790444965.139975\\
2.25	790444965.139975\\
2.25	775610905.379772\\
1.75	775610905.379772\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
2.75	778811518.589989\\
2.75	797440093.455926\\
3.25	797440093.455926\\
3.25	778811518.589989\\
2.75	778811518.589989\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
3.75	855321034.77516\\
3.75	874920787.999411\\
4.25	874920787.999411\\
4.25	855321034.77516\\
3.75	855321034.77516\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
4.75	857650560.681162\\
4.75	873518182.255416\\
5.25	873518182.255416\\
5.25	857650560.681162\\
4.75	857650560.681162\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
5.75	861788099.394419\\
5.75	880909562.089288\\
6.25	880909562.089288\\
6.25	861788099.394419\\
5.75	861788099.394419\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
0.75	781793836.105095\\
1.25	781793836.105095\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
1.75	780287401.760759\\
2.25	780287401.760759\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
2.75	788619384.720615\\
3.25	788619384.720615\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
3.75	864306297.354719\\
4.25	864306297.354719\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
4.75	862916397.251492\\
5.25	862916397.251492\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
5.75	871171882.066934\\
6.25	871171882.066934\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
1	823604884.762596\\
1	824554450.819763\\
1	824610155.741313\\
1	825641235.941777\\
1	825912384.550599\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
2	815188296.691335\\
2	816201389.414606\\
2	816424106.688419\\
2	817741202.104316\\
2	819991657.83441\\
2	820192059.578569\\
2	823150222.18846\\
2	823604884.762596\\
2	824554450.819763\\
2	825490307.477738\\
2	825641235.941777\\
2	825912384.550599\\
2	826395496.03145\\
2	840726149.312338\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
3	825472889.757102\\
3	825490307.477738\\
3	825641235.941777\\
3	825912384.550599\\
3	826395496.03145\\
3	840726149.312338\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
4	904346329.899738\\
4	905251653.679862\\
4	906239304.248086\\
4	908068570.845574\\
4	910367766.627328\\
4	911358091.190934\\
4	916485703.368503\\
4	918012824.259251\\
4	924868564.865786\\
4	925018898.010505\\
4	929105395.58096\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
5	900971625.51047\\
5	903573276.276988\\
5	905251653.679862\\
5	905960916.427505\\
5	906239304.248086\\
5	906633491.800299\\
5	907859968.754162\\
5	908068570.845574\\
5	910367766.627328\\
5	911358091.190934\\
5	916485703.368503\\
5	918012824.259251\\
5	918162771.147715\\
5	924868564.865786\\
5	925018898.010505\\
5	929105395.58096\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
6	831066944.384475\\
6	910367766.627328\\
6	911010354.414058\\
6	911358091.190934\\
6	916485703.368503\\
6	918012824.259251\\
6	918162771.147715\\
6	924868564.865786\\
6	929105395.58096\\
};
\end{axis}
\end{tikzpicture}%

==> Images/results/boxplots/boxplot_density16.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.8\linewidth,
height=1.0in,
at={(5in,0in)},
scale only axis,
xmin=0.5,
xmax=6.5,
xtick={1,2,3,4,5,6},
xticklabels={{SMURF-T}, {DBR-T}, {BASMURF-T},{SMURF},{DBR},{BASMURF}},
xticklabel style={rotate=45},
ymin=750732521.435512,
ymax=956036765.721589,
ylabel style={font=\color{white!15!black}},
ylabel={average throughput},
xlabel={(b) $Density = 40000~UAVs/km^3$},
axis background/.style={fill=white},
title style={font=\bfseries},
% title={Boxplot of average throughput with H=16}
]
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	795887919.699088\\
1	826507187.018711\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	790330857.737537\\
2	810317395.103733\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	801571647.139812\\
3	822119129.269498\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	877307216.007575\\
4	907410979.06294\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	873666284.57471\\
5	896855685.343253\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	884212013.816386\\
6	905941589.375532\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	760064532.539425\\
1	774668757.050829\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	769078528.519686\\
2	775959332.952444\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	764401952.066726\\
3	786528407.605069\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	840777425.927804\\
4	856956237.770768\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	851933721.60935\\
5	857971638.549025\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	848913637.250784\\
6	869342062.837697\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	826507187.018711\\
1.125	826507187.018711\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	810317395.103733\\
2.125	810317395.103733\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	822119129.269498\\
3.125	822119129.269498\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	907410979.06294\\
4.125	907410979.06294\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	896855685.343253\\
5.125	896855685.343253\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	905941589.375532\\
6.125	905941589.375532\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	760064532.539425\\
1.125	760064532.539425\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	769078528.519686\\
2.125	769078528.519686\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	764401952.066726\\
3.125	764401952.066726\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	840777425.927804\\
4.125	840777425.927804\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	851933721.60935\\
5.125	851933721.60935\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	848913637.250784\\
6.125	848913637.250784\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
0.75	774668757.050829\\
0.75	795887919.699088\\
1.25	795887919.699088\\
1.25	774668757.050829\\
0.75	774668757.050829\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
1.75	775959332.952444\\
1.75	790330857.737537\\
2.25	790330857.737537\\
2.25	775959332.952444\\
1.75	775959332.952444\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
2.75	786528407.605069\\
2.75	801571647.139812\\
3.25	801571647.139812\\
3.25	786528407.605069\\
2.75	786528407.605069\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
3.75	856956237.770768\\
3.75	877307216.007575\\
4.25	877307216.007575\\
4.25	856956237.770768\\
3.75	856956237.770768\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
4.75	857971638.549025\\
4.75	873666284.57471\\
5.25	873666284.57471\\
5.25	857971638.549025\\
4.75	857971638.549025\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
5.75	869342062.837697\\
5.75	884212013.816386\\
6.25	884212013.816386\\
6.25	869342062.837697\\
5.75	869342062.837697\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
0.75	782618003.583425\\
1.25	782618003.583425\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
1.75	780049673.72733\\
2.25	780049673.72733\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
2.75	793815167.036582\\
3.25	793815167.036582\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
3.75	864729063.900332\\
4.25	864729063.900332\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
4.75	862550464.859822\\
5.25	862550464.859822\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
5.75	875174479.893472\\
6.25	875174479.893472\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
1	828359001.311907\\
1	833912271.011185\\
1	834946707.03586\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
2	811939551.552759\\
2	811984482.912331\\
2	813369632.153778\\
2	813544124.547294\\
2	813812046.384688\\
2	814017517.370102\\
2	815275317.747057\\
2	815760799.703124\\
2	817469959.322292\\
2	818335324.254775\\
2	818378494.499514\\
2	820303211.701598\\
2	821037324.547631\\
2	821159891.141692\\
2	821657409.550337\\
2	822119129.269498\\
2	824404458.869539\\
2	824733074.565853\\
2	825356906.84688\\
2	828359001.311907\\
2	833912271.011185\\
2	834946707.03586\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
3	824404458.869539\\
3	824733074.565853\\
3	825356906.84688\\
3	826507187.018711\\
3	828359001.311907\\
3	833912271.011185\\
3	833971865.608401\\
3	834946707.03586\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
4	909781460.74685\\
4	912252152.619715\\
4	913014382.429233\\
4	913287284.415689\\
4	914129886.544792\\
4	915446350.89035\\
4	915917663.172048\\
4	946704754.617676\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
5	897401659.388117\\
5	897803099.448216\\
5	899200987.702071\\
5	901504726.712674\\
5	904088065.777117\\
5	905538289.994172\\
5	905721566.727783\\
5	905941589.375532\\
5	907410979.06294\\
5	909969391.878354\\
5	912252152.619715\\
5	913014382.429233\\
5	913287284.415689\\
5	914129886.544792\\
5	915446350.89035\\
5	915917663.172048\\
5	916466791.640952\\
5	946704754.617676\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
6	906796138.040119\\
6	907410979.06294\\
6	909781460.74685\\
6	909969391.878354\\
6	911156586.294797\\
6	912252152.619715\\
6	913014382.429233\\
6	913287284.415689\\
6	914129886.544792\\
6	915446350.89035\\
6	915917663.172048\\
6	916466791.640952\\
6	946704754.617676\\
};
\end{axis}
\end{tikzpicture}%

==> Images/results/boxplots/boxplot_density24.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.8\linewidth,
height=1.0in,
at={(0in,1.5in)},
scale only axis,
xmin=0.5,
xmax=6.5,
xtick={1,2,3,4,5,6},
xticklabels={{SMURF-T}, {DBR-T}, {BASMURF-T},{SMURF},{DBR},{BASMURF}},
xticklabel style={rotate=45},
ymin=748329466.075407,
ymax=954627999.845576,
ylabel style={font=\color{white!15!black}},
ylabel={average throughput},
xlabel={(c) $Density = 60000~UAVs/km^3$},
axis background/.style={fill=white},
title style={font=\bfseries},
% title={Boxplot of average throughput with H=24}
]
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	793108059.265215\\
1	817752561.55979\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	788641123.714822\\
2	806599427.301925\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	803976611.091435\\
3	822912416.717821\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	877399640.765094\\
4	900659316.624521\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	872931220.142377\\
5	893755262.54883\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	887718296.216651\\
6	908039351.19763\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	757706672.155869\\
1	776363722.968453\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	763554423.693555\\
2	776626035.120499\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	772510478.181246\\
3	791168473.447888\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	841919612.191916\\
4	859096258.04805\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	851607900.82576\\
5	858837581.712018\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	857102746.447137\\
6	873314025.417982\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	817752561.55979\\
1.125	817752561.55979\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	806599427.301925\\
2.125	806599427.301925\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	822912416.717821\\
3.125	822912416.717821\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	900659316.624521\\
4.125	900659316.624521\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	893755262.54883\\
5.125	893755262.54883\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	908039351.19763\\
6.125	908039351.19763\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	757706672.155869\\
1.125	757706672.155869\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	763554423.693555\\
2.125	763554423.693555\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	772510478.181246\\
3.125	772510478.181246\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	841919612.191916\\
4.125	841919612.191916\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	851607900.82576\\
5.125	851607900.82576\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	857102746.447137\\
6.125	857102746.447137\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
0.75	776363722.968453\\
0.75	793108059.265215\\
1.25	793108059.265215\\
1.25	776363722.968453\\
0.75	776363722.968453\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
1.75	776626035.120499\\
1.75	788641123.714822\\
2.25	788641123.714822\\
2.25	776626035.120499\\
1.75	776626035.120499\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
2.75	791168473.447888\\
2.75	803976611.091435\\
3.25	803976611.091435\\
3.25	791168473.447888\\
2.75	791168473.447888\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
3.75	859096258.04805\\
3.75	877399640.765094\\
4.25	877399640.765094\\
4.25	859096258.04805\\
3.75	859096258.04805\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
4.75	858837581.712018\\
4.75	872931220.142377\\
5.25	872931220.142377\\
5.25	858837581.712018\\
4.75	858837581.712018\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
5.75	873314025.417982\\
5.75	887718296.216651\\
6.25	887718296.216651\\
6.25	873314025.417982\\
5.75	873314025.417982\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
0.75	783714273.094461\\
1.25	783714273.094461\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
1.75	781576575.53077\\
2.25	781576575.53077\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
2.75	797464767.820964\\
3.25	797464767.820964\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
3.75	866725398.998978\\
4.25	866725398.998978\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
4.75	863948453.804145\\
5.25	863948453.804145\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
5.75	880267932.853039\\
6.25	880267932.853039\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
1	818435266.493\\
1	822275132.188976\\
1	826020985.34495\\
1	826133688.992798\\
1	826227647.067153\\
1	830869192.847482\\
1	832961513.392311\\
1	833352649.64905\\
1	833981099.655817\\
1	835711425.813973\\
1	835765415.830221\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
2	806987390.932397\\
2	810183436.739867\\
2	810795671.283063\\
2	815214403.437059\\
2	817752561.55979\\
2	818435266.493\\
2	822275132.188976\\
2	826020985.34495\\
2	826133688.992798\\
2	826227647.067153\\
2	830869192.847482\\
2	832961513.392311\\
2	833352649.64905\\
2	833981099.655817\\
2	835711425.813973\\
2	835765415.830221\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
3	770142253.028775\\
3	824726393.363364\\
3	826133688.992798\\
3	827712885.356653\\
3	832809753.742724\\
3	832961513.392311\\
3	833352649.64905\\
3	833981099.655817\\
3	835711425.813973\\
3	835765415.830221\\
3	836486492.508948\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
4	906746444.073011\\
4	908039351.19763\\
4	911004927.593244\\
4	912119067.235154\\
4	913322094.39454\\
4	914779736.890289\\
4	915790080.431812\\
4	921511913.866226\\
4	923491754.082368\\
4	935002162.047822\\
4	936268813.045457\\
4	940286573.947251\\
4	945250793.765114\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
5	895427496.155924\\
5	895771747.400075\\
5	897354384.356025\\
5	900659316.624521\\
5	904797326.3571\\
5	908039351.19763\\
5	911004927.593244\\
5	912119067.235154\\
5	913322094.39454\\
5	914779736.890289\\
5	915790080.431812\\
5	921511913.866226\\
5	923491754.082368\\
5	935002162.047822\\
5	936268813.045457\\
5	940286573.947251\\
5	945250793.765114\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
6	910149133.249064\\
6	911004927.593244\\
6	911202677.364133\\
6	913322094.39454\\
6	913463335.459537\\
6	915790080.431812\\
6	917569437.5229\\
6	921511913.866226\\
6	923491754.082368\\
6	935002162.047822\\
6	936268813.045457\\
6	939363459.789328\\
6	945250793.765114\\
};
\end{axis}
\end{tikzpicture}%

==> Images/results/boxplots/boxplot_density30.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.8\linewidth,
height=1.0in,
at={(0in,1.5in)},
scale only axis,
xmin=0.5,
xmax=6.5,
xtick={1,2,3,4,5,6},
xticklabels={{SMURF-T}, {DBR-T}, {BASMURF-T},{SMURF},{DBR},{BASMURF}},
xticklabel style={rotate=45},
ymin=749745379.926311,
ymax=985543380.403469,
ylabel style={font=\color{white!15!black}},
ylabel={average throughput},
xlabel={(d) $Density = 75000~UAVs/km^3$},
axis background/.style={fill=white},
title style={font=\bfseries},
% title={Boxplot of average throughput with H=30}
]
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	794666315.727954\\
1	818414741.919468\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	787370193.73126\\
2	804084379.996114\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	805997114.294346\\
3	820153895.919076\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	876729114.235521\\
4	898412879.100149\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	870737299.636545\\
5	887410416.771279\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	889258227.280619\\
6	908082873.694638\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	760463470.857091\\
1	778710618.380795\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
2	767299095.241889\\
2	775986388.658281\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
3	781230751.407736\\
3	794896124.05621\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
4	846165266.92507\\
4	861651954.970379\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
5	852697130.195838\\
5	858357269.941981\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
6	858416762.146177\\
6	876533164.771971\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	818414741.919468\\
1.125	818414741.919468\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	804084379.996114\\
2.125	804084379.996114\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	820153895.919076\\
3.125	820153895.919076\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	898412879.100149\\
4.125	898412879.100149\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	887410416.771279\\
5.125	887410416.771279\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	908082873.694638\\
6.125	908082873.694638\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0.875	760463470.857091\\
1.125	760463470.857091\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1.875	767299095.241889\\
2.125	767299095.241889\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
2.875	781230751.407736\\
3.125	781230751.407736\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
3.875	846165266.92507\\
4.125	846165266.92507\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
4.875	852697130.195838\\
5.125	852697130.195838\\
};
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
5.875	858416762.146177\\
6.125	858416762.146177\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
0.75	778710618.380795\\
0.75	794666315.727954\\
1.25	794666315.727954\\
1.25	778710618.380795\\
0.75	778710618.380795\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
1.75	775986388.658281\\
1.75	787370193.73126\\
2.25	787370193.73126\\
2.25	775986388.658281\\
1.75	775986388.658281\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
2.75	794896124.05621\\
2.75	805997114.294346\\
3.25	805997114.294346\\
3.25	794896124.05621\\
2.75	794896124.05621\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
3.75	861651954.970379\\
3.75	876729114.235521\\
4.25	876729114.235521\\
4.25	861651954.970379\\
3.75	861651954.970379\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
4.75	858357269.941981\\
4.75	870737299.636545\\
5.25	870737299.636545\\
5.25	858357269.941981\\
4.75	858357269.941981\\
};
\addplot [color=blue, forget plot]
  table[row sep=crcr]{%
5.75	876533164.771971\\
5.75	889258227.280619\\
6.25	889258227.280619\\
6.25	876533164.771971\\
5.75	876533164.771971\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
0.75	786246616.066044\\
1.25	786246616.066044\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
1.75	780575338.313849\\
2.25	780575338.313849\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
2.75	799959995.118811\\
3.25	799959995.118811\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
3.75	869303980.203425\\
4.25	869303980.203425\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
4.75	862772603.90747\\
5.25	862772603.90747\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
5.75	882457592.893627\\
6.25	882457592.893627\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
1	821827945.259644\\
1	822064173.375343\\
1	825436819.748656\\
1	825496832.255151\\
1	830669576.327232\\
1	830831417.078805\\
1	831328954.580895\\
1	832127107.719036\\
1	832525725.600518\\
1	837369685.514345\\
1	846466399.211873\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
2	806957107.557953\\
2	808320276.068811\\
2	808469856.373882\\
2	813459245.738067\\
2	813790363.555045\\
2	814165346.599326\\
2	815732121.498907\\
2	815867115.770564\\
2	817001131.980086\\
2	818414741.919468\\
2	820153895.919076\\
2	822064173.375343\\
2	825436819.748656\\
2	825496832.255151\\
2	830669576.327232\\
2	830831417.078805\\
2	831328954.580895\\
2	832127107.719036\\
2	832525725.600518\\
2	837369685.514345\\
2	846466399.211873\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
3	771863576.544481\\
3	822739071.268847\\
3	825436819.748656\\
3	825496832.255151\\
3	827975227.936891\\
3	830669576.327232\\
3	830831417.078805\\
3	831328954.580895\\
3	832127107.719036\\
3	832525725.600518\\
3	837369685.514345\\
3	846466399.211873\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
4	906298434.346239\\
4	906719653.019169\\
4	907502706.490384\\
4	910378468.582667\\
4	910949624.949905\\
4	912344254.779563\\
4	913293805.247172\\
4	914901515.031206\\
4	916311719.763073\\
4	916372494.55165\\
4	918543713.756735\\
4	925164616.065377\\
4	931079637.273574\\
4	974825289.472689\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
5	892360658.217547\\
5	894287163.407346\\
5	894699663.908591\\
5	895577977.294179\\
5	897331026.413707\\
5	898412879.100149\\
5	906298434.346239\\
5	906719653.019169\\
5	907502706.490384\\
5	910378468.582667\\
5	910949624.949905\\
5	912344254.779563\\
5	913293805.247172\\
5	914901515.031206\\
5	916311719.763073\\
5	916372494.55165\\
5	918543713.756735\\
5	925164616.065377\\
5	931079637.273574\\
5	974825289.472689\\
};
\addplot [color=black, only marks, mark=+, mark options={solid, draw=red}, forget plot]
  table[row sep=crcr]{%
6	909014666.905396\\
6	910378468.582667\\
6	910949624.949905\\
6	911051525.773745\\
6	913293805.247172\\
6	914901515.031206\\
6	916311719.763073\\
6	918543713.756735\\
6	925164616.065377\\
6	931079637.273574\\
6	974825289.472689\\
};
\end{axis}
\end{tikzpicture}%
